Planning the path with Reinforcement Learning: Optimal Robot Motion Planning in RoboCup Small Size League Environments

This work investigates the potential of Reinforcement Learning (RL) to tackle robot motion planning challenges in the dynamic RoboCup Small Size League (SSL). Using a heuristic control approach, we evaluate RL's effectiveness in obstacle-free and single-obstacle path-planning environments. Ablation studies reveal significant performance improvements. Our method achieved a 60% time gain in obstacle-free environments compared to baseline algorithms. Additionally, our findings demonstrated dynamic obstacle avoidance capabilities, adeptly navigating around moving blocks. These findings highlight the potential of RL to enhance robot motion planning in the challenging and unpredictable SSL environment.

==> content/acknowledgement.tex <==
\section{Acknowledgement}

We would like to first thanks to our advisors and the Informatic Center - UFPE (Centro de Informática (CIn) - UFPE) for all the support and knowledge during this year of project and development. We also would like to thanks all the help from our sponsors: Incognia, Cesar, Embraer, HSBS, Instituto Nacional de .
